To Burst or Not to Burst: Generating and Quantifying Improbable Text

While large language models (LLMs) are extremely capable at text generation, their outputs are still distinguishable from human-authored text. We explore this separation across many metrics over text, many sampling techniques, many types of text data, and across two popular LLMs, LLaMA and Vicuna. Along the way, we introduce a new metric, recoverability, to highlight differences between human and machine text; and we propose a new sampling technique, burst sampling, designed to close this gap. We find that LLaMA and Vicuna have distinct distributions under many of the metrics, and that this influences our results: Recoverability separates real from fake text better than any other metric when using LLaMA. When using Vicuna, burst sampling produces text which is distributionally closer to real text compared to other sampling techniques.

==> average_metric_separability.tex <==
\begin{table}
\small
\centering
\begin{tabular}{| l | r r |}
\hline
\textbf{Metric} & \textbf{LLaMA} & \textbf{Vicuna}\\
\hline
k burst & 0.341 & 0.525\\
p burst & 0.372 & 0.813\\
top-p burst & 0.392 & 0.206\\
log-likelihood & 0.467 & \textbf{0.855}\\
log rank & 0.458 & 0.820\\
rank & 0.317 & 0.349\\
perplexity & 0.467 & \textbf{0.855}\\
diversity & 0.433 & 0.417\\
recov top k=40 & \textbf{0.524} & 0.765\\
recov top k=50 & 0.522 & 0.743\\
\hline
\end{tabular}
\caption{\label{average_metric_sep_table}For each metric, average separation between distributions of metric values for real and generated text, across all datasets and sampling methods. The \emph{highest} value is highlighted in each column, indicating that the given metric is the best, on average, at providing a distinction between real and synthetic text.}
\end{table}

==> average_metrics.tex <==
\begin{table}
\small
\centering
\begin{tabular}{| l | c c |}
\hline
\textbf{Metric} & \textbf{LLaMA} & \textbf{Vicuna}\\
\hline
k burst & 7.869 & 9.673\\
p burst & 0.863 & 0.577\\
top-p burst & 0.363 & 0.241\\
log-likelihood & -1.887 & -1.211\\
log rank & 0.851 & 0.503\\
rank & 39.978 & 39.799\\
perplexity & 9.475 & 4.736\\
diversity & 0.795 & 0.781\\
recov top k=40 & 0.946 & 0.966\\
recov top k=50 & 0.953 & 0.970\\
\hline
\end{tabular}
\caption{\label{average_metrics_table}Average metrics for generated text across all datasets and sampling methods.}
\end{table}
